Higher-Order Contributions in Higgs Sectors of Supersymmetric Models

In 2012, the discovery of a particle compatible with a Higgs boson of a mass of roughly 125 GeV was announced. This great success is now being followed by the identification of the nature of this particle and the particle's properties are being measured. One of these properties is the Higgs boson mass which is already known very precisely with an experimental uncertainty of below 1 GeV. In some extensions of the Standard Model, like in supersymmetric extensions, the Higgs boson mass can be predicted and hence, the measured mass constrains the parameters of the model. For a full exploitation of this constraint, a precise theoretical prediction is needed. The presented combination of the results obtained by the Feynman diagrammatic approach and the renormalization group equation approach improves the known Higgs mass prediction for larger mass scales of the superpartner particles.

==> preprint.tex <==
FR-PHENO-2014-007\\
MPP-2014-262
%arXiv:1407.nnnn [hep-ph]

